aLEAKator: HDL Mixed-Domain Simulation for Masked Hardware \& Software Formal Verification

Verifying the security of masked hardware and software implementations, under advanced leakage models, remains a significant challenge, especially then accounting for glitches, transitions and CPU micro-architectural specifics. Existing verification approaches are either restricted to small hardware gadgets, small programs on CPUs such as Sboxes, limited leakage models, or require hardware-specific prior knowledge. In this work, we present aLEAKator, an open-source framework for the automated formal verification of masked cryptographic accelerators and software running on CPUs from their HDL descriptions. Our method introduces mixed-domain simulation, enabling precise modeling and verification under various (including robust and relaxed) 1-probing leakage models, and supports variable signal granularity without being restricted to 1-bit wires. aLEAKator also supports verification in the presence of lookup tables, and does not require prior knowledge of the target CPU architecture. Our approach is validated against existing tools and real-world measurements while providing innovative results such as the verification of a full, first-order masked AES on various CPUs

==> includes/6-review.tex <==

\newpage

\section*{Major Revision}

As instructed in the major revision notice, the following section is dedicated to answer how the requests made by the reviewers have been addressed and what modifications were introduced to the submission. The previous review discussion is given in the first subsection, we then discuss the modifications introduced and conclude with the previous and current long-paper approval.

{\rb We want to notice reviewers that all benchmarks from~\ref{tb:results-sw} have been re-run. The version of the \tool{Secmult-nsec} on the Cortex-M3 and M4 were not the same as the ones run for the t-tests in Figures~\ref{fig:secmult-m3-unsecure} and ~\ref{fig:secmult-m4-unsecure}, which was a mistake (wrong verified binary) for which we apologize. Also, subsequent developments of \framework{} led to more optimisations so the results are overall better in time. }

\subsection*{Revision Requirements}

We tried, to the best extent, to indicate in {\rv red text} all text modifications in the current submission. We provide in the supplementary materials both the non-annotated version of this submission and the previously submitted version.

The major modification requirements are split in four points which we addressed the following way:

%%KH-GPT We have made every effort to highlight all textual changes in this submission using {\rb red text}. In the supplementary materials, we provide both a clean (non-annotated) version of this submission as well as the previously submitted version.

The primary points raised for major modifications are as follows, and we addressed them in these ways:

\begin{mdframed}[rightline=false, topline=false, bottomline=false]
- Include more results to showcase the matches between the leakages observed in practice and the leakages detected by aLEAKator, for at least two chosen algorithms
\end{mdframed}

{\rb We have added Section 5.2.5, which offers a cycle-accurate comparison between the output from \framework{} and t-test measurements for three programs executed on a Cortex-M4 core. This section demonstrates that no practical leakage occurs without a corresponding detection by \framework{} and offers explanations for cases where the matches are not perfect. }

\begin{mdframed}[rightline=false, topline=false, bottomline=false]
- Include a case-example of a program on a given CPU detailing main leakage sources, together with a discussion
\end{mdframed}

{\rb In the newly added Section 5.2.5, we include an in-depth analysis of the typical sources of leakage for each program running on the Cortex-M4 and discuss why \framework{} identifies them as such, based on the definitions in the relevant section. Additionally, we introduce a benchmark, called "refresh", to illustrate a very subtle leakage and show how \framework{} allows for precise identification of its root cause. }

\begin{mdframed}[rightline=false, topline=false, bottomline=false]
- Elaborate how aLEAKator can be extended to another use cases e.g. to provide the needed information for verifMSI and to other leakage properties such as PINI etc.
\end{mdframed}

{\rb We have added a Section 5.3 to show that \framework{} is able to handle other security properties. Results on the NI and SNI properties are given to support this claim and their benchmarks will also be made open-source at publication time. We also discuss how other properties could be supported.}

\begin{mdframed}[rightline=false, topline=false, bottomline=false]
- Provide a more detailed discussion on possible extensions, and lack thereof, to higher orders.
\end{mdframed}

{\rb We also added in Section 5.3 a discussion on how \framework{} can also handle higher-order, how it is currently considered by state-of-the-art tools, and we reproduce some results for the spatial higher-order on hardware gadgets. We also provide insight on the intrinsic limitation of verifying higher-order.}

%% KH-GPT proposition {\rb Section 5.3 has been expanded to show that \framework{} also addresses higher-order scenarios. We explain how current state-of-the-art tools treat this aspect and we replicate their results for spatial higher-order leakages on hardware gadgets. Moreover, we discuss inherent limitations in verifying higher-order properties. Benchmark results for higher-order cases will also be made available as open source.}

\subsection*{Minor Changes in the Revision}

We tried to exhaustively address all remarks and typos reported in the reviews. This section is dedicated to explain the most significant changes amongst them.

{\rb Review \#7A: We have rephrased line 118 to better explain that the verification of a property can be done in more or less "sub-verifications" depending on optimisations. }

{\rb Typos from (old version) lines 277, 315, 332, 342, 345, 391, 644 as well as Table 5 have been corrected. }

{\rb Review \#7B: The unclear definitions that could refer to a negative cycle number have been corrected to better reflect that the initial state and all input sequences lead to a defined value for all wires (equations 7, 8, 9, 10 and 11). Related to this topic, we hope to have addressed in a clearer way how the definitions of the evaluation functions do not lead to a circular definition. }

{\rb Review \#7B: We clarified line 62 how the RR d-probing model is different from the (1,1) d-probing model. We have also added a reference line 205 to illustrate how enumeration can be used to verify expressions.}

{\rb Review \#7B: We better explained why no results are given for \prover{} and \prolead{} on some hardware benchmarks in Table~\ref{tb:res-implem-hw}. We also clarified units (GB) and explained the different cycles columns meanings. }

{\rb Review \#7B: We have highlighted in lines 317 and 377 that the nature of handled data is given as an input. In line 377 we emphasize that the constructed expressions during simulation represent the computation performed with input data, and that the nature of this data does not change the computation. The exact nature of each symbolic variable is necessary at verification time and not at simulation time.}

{\rb Review \#7C: Major requested changes have been integrated, c.f. previous section.}

\newpage

\subsection*{Previous Review}
Paper \#7 Long Paper: aLEAKator: HDL Mixed-Domain Simulation for Masked
Hardware \& Software Formal Verification

\subsubsection*{Review \#7A}
* Updated: Sep 13, 2025, 9:56:43 AM UTC

\noindent Overall merit: 4. Minor Revision (MinR)

\noindent Relevance to TCHES: 3. Right in the middle of CHES

\noindent Novelty/Contribution: 3. Major Contribution

\noindent Reviewer expertise: 3. I am knowledgeable in this subfield but not expert (I know some related
   works and may have a publication in the subfield)

\noindent Confidence: 2. Medium

\noindent Editorial quality: 4. Well-written

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Paper summary:

The paper proposes a more scalable approach to validate probing security properties in cryptographic circuits or in cryptographic software running on a microprocessor. This is achieved by "mixed-domain simulation", where in addition to actual logical or integer values being processed, a number of propagation-related data is computed and processed. Specifically, the abstracted description of the masking scheme used for protection; glitch-aware information-leakage conditions; and signal-stability properties for refined analysis in some of the probing models. The resulting framework is announced to be made open-source upon acceptance.

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Strengths:

+ Automated procedure for arbitrary circuits and different probing models.

+ Improved performance compared to earlier approaches.

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Weaknesses:

- I find naming "formal verification" unfortunate, as the procedure is, despite producing symbolic information, based on a specific inmput sequence, whereas "true" formal verification methods should be universal for all sequences. I do see that this is how comparable approaches are called in prior work and have no better suggestion.

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Comments for authors:

98: Illogical sentence (why is considering or not microarchitecture lead to more or less security? I can imagine that it is easier or harder to validate security, but the "amount" of security itself shoudl not depend on what the verifier is looking at).

118: "number of verification" sounds strange to me; either a property hold, and then one "verification" is sufficient, or it maybe holds with probabilty and having more is better, but then I would call it "validation", not "verification". Same comnment regarding "eight formal verifications" in 128.

\newpage

\subsubsection*{Review \#7B}
* Updated: Sep 6, 2025, 3:00:02 PM UTC

\noindent Overall merit: 3. Major Revision (MajR)

\noindent Relevance to TCHES: 3. Right in the middle of CHES

\noindent Novelty/Contribution: 2. Minor Contribution

\noindent Reviewer expertise: 1. I don't know this subfield

\noindent Confidence: 1. Low (will defer to experts)

\noindent Editorial quality: 3. Adequate

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Paper summary:

A new leakage model called d-sw-probing model is proposed in this
paper. A characteristic of the new leakage model is the explicit
probe width, which allows verification of hardware circuits at gate
level, and software implementations executing on CPUs. The new leakage
model is implemented in the tool aLEAKator, which collects data (as
symbolic expressions) from the model simulation and then relies on
the external tool VerifMSI++ to verify security properties. The
experimental results show that aLEAKator outperforms CoCo, Prover,
and Prolead. The experimental results also show the performance
of aLEAKator in verifying software implementations on various CPUs.
The results of verifying software implementations are validated
using real power measurements.

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Strengths:

- A flexible model supporting both hardware circuits and software
  implementations
  
- An implementation is available

- Some verification results are validated

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Weaknesses:

- The model is an over-approximation which may results in false
  positives
  
- Limited to RR 1-sw-probing model

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Comments for authors:

One advantage of using symbolic expressions is that falling back
to enumeration is possible when verification cannot conclude for
a small expression. From an over-approximation (of the expressions to be verified) back to a full
enumeration is a big jump. I wonder if the abstraction level (regarding the expressions)
can be made configurable. Moreover, in model checking, there is
a technique called CEGAR (Counter-Example Guided Abstraction
Refinement) [1,2], which uses spurious counterexamples to refine
abstract models, so that both efficiency and precision can be
guaranteed. If various abstraction levels are available, then
such refinement technique may work for the leakage model.
Note that what's analogous to an abstract model here is the set of expressions to be verified.

[1] https://en.wikipedia.org/wiki/Counterexample-guided\_abstraction\_refinement

[2] Edmund Clarke, Orna Grumberg, Somesh Jha, Yuan Lu, Helmut Veith.
    Counterexample-guided abstraction refinement for symbolic model checking.
    Journal of the ACM. 50 (5): 752–794.

One feature of aLEAKator is the support of lookup tables, but
I didn't find how lookup tables are supported. The short
description about reading from a table at line 845 may be
relevant. I'm curious about the difficulty of supporting lookup
tables.

- Line 277: advantages => advantage

- Line 288: There are variants of d-sw-probing model, including

  + d-sw-probing model (line 250)
  
  + (g, t) d-sw-probing model (line 54)
  
  + RR 1-sw-probing model (line 288)
  
  I am confused by (1, 1) 1-sw-probing model and RR 1-sw-probing
  model. Are they the same?
  
- Line 301: Symbolic expressions describe wire values with respect
  to sensitive information such as shares, secrets, and masks. It
  would be good to have more details about how sensitive information
  is described by symbolic expressions defined in line 386.
  
- Line 315: describes => describe

- Line 332: are modelled => is modelled

- Line 342: Replace "gate g" with "gate r" to match the suffix of
  w\_r\^{}{in} and w\_r\^{}{out}.
  
- Line 345: an example of circuit => an example of a circuit

- Line 345: types of gate => types of gates

- Lines 407, 419, and 436: The font of w and t in eval(w, t)
  here is inconsistent to the font in Equation 7. Is this intended?
  
- Lines 404 and 409: By line 404, the valuation {}\^{}{c}\textbackslash alpha\_w\^{}t
  (included in \textbackslash alpha\_w\^{}t) is computed with the application of an
  evaluation function (which is supposed to be eval). By Equation
  7 at line 409, the evaluation function eval is defined by
  {}\^{}{c}\textbackslash alpha\_w\^{}t for the first case. This results in a circular
  definition. The question is whether {}\^{}{c}\textbackslash alpha\_w\^{}t and
  {}\^{}{e}\textbackslash alpha\_w\^{}t are provided by the input stimuli for all
  w \textbackslash  in I and for all t. Please elaborate on what is contained
  in the input stimuli and fix the circular definition accordingly.
  
- Line 424: Define the term "equivalent".

- Line 434:

  + According to line 391, stability domain is a set of Boolean
    vectors. The first case is a Boolean, not a Boolean vector.
    
  + The description in line 424 uses the term "equivalent" but
    an equality symbol is used in the second case. The mapping
    from equality (or equivalence) to stability domain is also
    unknown.
    
  + The granularity (symbolic expressions as a whole) of the
    second case and the granularity (down to bits according to
    Table 4) of the third case seem to be different. Please explain.
    
  + According to the Inputs column in Table 4, the symbolic
    evaluation {}\^{}{e}eval(w\_i, t) is not always required by
    {}\^{}{s}f\_g. But in Equation 9, {}\^{}{e}eval(w\_i, t) is always
    passed as an argument.
    
- Table 4: The access to i-th bit of a symbolic expression is used
  here. I wonder how this is done and what is the precision.
  Assume e1 is a symbolic expression of width n and e2 is e1
  shifted to the left by some constant m (0 < m < n). Does the
  computation know that e2[0] is 0?
  
- Line 453: Footnote 4 states that trivial sets are defined as an
  empty sets. Please consider another way to define the sets by
  subtracting all constants from the set in Equation 10 (or do
  the subtraction in another new equation).
  
- Table 5: add a space before "if"

- Algorithm 2: EVAL(r, 0) with r \textbackslash in R returns \textbackslash alpha\_{w\_g\^{}in}\^{}{-1},
  which is not defined.
  
- Table 7: in the wires to verify for the (1,0) 1-sw-probing model,
  the stability of a wire should be a Boolean vector of some width,
  not a tuple <0>.
  
- Line 513 and Table 7: MUX is never mentioned before.

- Line 636: What is the unit Go? Is it same as GB (gigabyte)?

- Table 10:

  + There are two numbers in the Cycles column for each masked
    hardware. What does the second number mean?
    
  + Explain why there are "-" results under Prover and Prolead.
  
- Line 644: RR 1 bit-probing => RR 1-bit-probing

- Line 649: maskVerif is not shown in Table 10

- Line 652: What is exactly the enumeration? If this is already
  explained somewhere, please make a clear reference.
  
- Line 675: When the analysis of aLEAKator results in a false
  positive, does aLEAKator produce any information for further
  debugging?
  
- Line 746: What is SBox[i]?

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Questions for authors’ response:

Do you think the CEGAR technique (mentioned in the comment) is
applicable to refining the leakage model?

How difficult is it to present a mix-domain simulation for RR
d-sw-probing model? This would make the presentation more complex
but would be more powerful.

\newpage

\subsubsection*{Review \#7C}

\noindent Overall merit: 3. Major Revision (MajR)

\noindent Relevance to TCHES: 3. Right in the middle of CHES

\noindent Novelty/Contribution: 3. Major Contribution

\noindent Reviewer expertise: 4. I work right in this subfield (I am well-versed with the related
   literature and publish regularly in the subfield)

\noindent Confidence: 3. High (will try to convince others)

\noindent Editorial quality: 4. Well-written

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Paper summary:

This work presents yet another tool for formal verification of masked cryptographic implementation and is suitable for both, hardware and software, including multiple CPUs.
The framework is proposed for the automated verification that is open-source and very efficient as it is able to verify a complete masked AES implementation in matter of minutes.

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Strengths:

- The topic is relevant and there is an important improvement from the state of the art tools

- The approach is verified on multiple CPUs, so it does not require any prior knowledge of the target CPU architecture

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Weaknesses:

- It works only for 1st order masking

- The evaluation presented in the paper is limited

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Comments for authors:

This is an important work and the fact that it is not CPU-specific makes it a very strong candidate to handle diverse architectures. It is introduced well and the write up and experiments are very helpful in understanding the tool's advantages compared to other related works.
I believe that this is a substantial contribution to this important topic of formal verification of protected implementations in hardware and software.

However, I still have some concerns that should be addressed before the work is published as follows:

- Table 11 is missing more details wrt leak cycles. There should be a check with actual traces showing that the PoIs are identified with the tool.

- The precision of the tool is not refined enough i.e. it only verified yes or no answers so far, a more insight in what exactly leak is missing.

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent Questions for authors’ response:

- How limited is the tool so far in its ability to handle different ciphers? As all the experiments are done with block ciphers, is there a problem to handle e.g. PQC algorithms?

- What was the reason to choose those 3 ciphers in Sect. 5.1?

- What are the bottleneck for adding higher-order verification and other models?

\newpage

\subsubsection*{Rebuttal Response by Author (532 words)}
Thank you very much for the highly valuable feedback. We will address, for the camera-ready version, the detailed comments and typos. 

Review C:
Table 11: We did not show the POIs for the sake of space, but we can provide for the camera-ready version more results to showcase the matches between the leakages observed in practice and the leakages detected by aLEAKator.

Precision: aLEAKator provides, for each detected leakage, much information for further debugging (cf. line 576+) : software instruction, CPU state, cycle number, HDL source wire name and line, leaking expression/set, etc. We did not provide precise leakage wire names in the paper because the list grows quickly. However, aLEAKator outputs have been used to remove leakage of the secured benchmarks presented in Table 11, highlighting the output precision. We can provide, for the camera-ready version, a case-example of a program on a given CPU detailing principal leakage sources. 

Selected ciphers: Ciphers in Section 5.1 have been chosen because they are implementations already verified by state-of-the-art tools. In particular, we showcased implementations for which CoCo, against which we aimed to compare aLEAKator, provides a verification verdict.

Masked PQC algorithms usually use additive masking. We think the latter could be handled by the verification manager, provided the verification tool, VerifMSI in our case, can handle such expressions (which would require a few additions).  Yet, the main challenge with PQC would be the number of cycles, which might induce huge expressions to verify. While we did not focus on such algorithms yet, we plan to do so in the future.
Regarding other leakage properties (PINI, SNI, ...), they are yet to be defined for software. For hardware implementations, aLEAKator can easily be extended to provide the needed information for verifMSI to perform such verifications, which are already implemented internally. However, aLEAKator has primarily been designed for verifying masked software running on CPU.

Reviews B and C:
Higher-order: We chose to focus on first order in this paper, and discussed about higher-order and limitations in lines 830+. We emphasized that all needed values for d-order verification are already computed, and that only the enumeration of d-uplets has not been implemented. The reason is that even at order 2, software verification results in a large number of combinations which does not scale (16M verifications for a single cycle of execution on a CPU with 4000 wires). We can provide a more detailed discussion in the final version.

Reviews B and A:
The verification of expressions does not rely on model-checking algorithms.

Additionally, for Review B, we did not consider CEGAR. It would not be applicable neither for enumeration nor for hardening since the initial program to be hardened is not an abstraction of the hardened one, the latter being another sequence of instructions guaranteeing a non-leaking execution. Moreover, even though a leakage in the 1-bit-probing-model implies a leakage in the 1-sw-probing-model, the latter is not an abstraction of the former but a stronger leakage model. The same relation applies between the different decompositions of the (g,t) 1-probing-models.

Input stimuli sequences are fixed and are composed of a valuation in each domain, thus there is no circular definition in practice. We will precise this in section 3.3.

\subsubsection*{Comment @A1 by Administrator}
Thank you for submitting your work to CHES 2026.  While the committee sees potential in the work, there are several issues that need to be fixed before the paper can be accepted.  As such, the committee invites you to submit a Major Revision.  The revision requirements are:

- Include more results to showcase the matches between the leakages observed in practice and the leakages detected by aLEAKator, for at least two chosen algorithms

- Include a case-example of a program on a given CPU detailing main leakage sources, together with a discussion

- Elaborate how aLEAKator can be extended to another use cases e.g. to provide the needed information for verifMSI and to other leakage properties such as PINI etc.

- Provide a more detailed discussion on possible extensions, and lack thereof, to higher orders.

\newpage

\subsection*{Previous Long-Paper Request}

\noindent On: Monday 7th of July 2025

\noindent To: ches2026programchairs@iacr.org, tches-managing-editor@iacr.org

\noindent Title: TCHES Volume 2026/1 - Long paper approval

\noindent Content:

Dear editors-in-chief and program chairs,

As mentioned on the TCHES submission webpage, we kindly ask you to
consider our submission entitled "aLEAKator: Formal Verification of
SW/HW Masked Implementations Using HDL Mixed-Domain Simulation", as a
long paper.

The paper currently spans 27 pages, and we believe that all the
contained material is essential for the paper to be complete and
self-contained. Specifically, the inclusion of formal definitions of our
approach, the implementation details, and the results are essential for
understanding and reproducibility.

The core of the paper consists of 8 pages dedicated to the formal
definition of our approach, accompanied by insightful examples, and 10
pages focused on implementation and experimental results. The remaining
pages provide context, background, and related work, which are equally
important for introducing our work and positioning it within the
existing research works.

Please find attached to this email a draft of the paper.

Could we kindly request your approval to submit our paper as a long
paper ?

Best regards,

[[author name, redacted]]

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent On: Monday 7th of July 2025

\noindent From: nele.mentens@kuleuven.be

\noindent Title: Re: TCHES Volume 2026/1 - Long paper approval 

\noindent Content:

Dear [[author name, redacted]],

We approve your request to submit a long paper as long as you stay within 25 pages.
Of course it is up to you to decide how to shrink to 25 pages, but it looks like there are many white spaces, lines with only a few words, and figures and tables that can be reduced in height.

Best regards,

Yuval and Nele


\newpage

\subsection*{Current Long-Paper Request}

\noindent On: Thursday 7th of October 2025

\noindent To: ches2026programchairs@iacr.org, tches-managing-editor@iacr.org

\noindent Title: TCHES Volume 2026/2 - Long paper re-approval 

\noindent Content:

Dear editors-in-chief and program chairs,

As mentioned on the TCHES submission webpage, we kindly ask you to consider our revised submission of "aLEAKator: Formal Verification of SW/HW Masked Implementations Using HDL Mixed-Domain Simulation", as a long paper.

Major revisions have been requested by the reviewers of the first volume of 2026 but we are not sure whether we need to ask again for an extension.

During the first volume, we were granted a 25 pages limit which we respected for the submission. For this volume, the following revisions have been requested:

    - Include more results to showcase the matches between the leakages observed in practice and the leakages detected by aLEAKator, for at least two chosen algorithms
    
    - Include a case-example of a program on a given CPU detailing main leakage sources, together with a discussion
    
    - Elaborate how aLEAKator can be extended to another use cases e.g. to provide the needed information for verifMSI and to other leakage properties such as PINI etc.
    
    - Provide a more detailed discussion on possible extensions, and lack thereof, to higher orders.

To address these required revisions with precision and rigor, we had to extend our results and discussion sections. The paper currently spans 30 pages and we would like to extend our current explanations (not present in the draft yet) to 31 pages.

Please find attached to this email a draft of the paper.

Could we kindly request your approval to submit our revised paper as a long paper ?
Best regards,

[[author name, redacted]]

\noindent\makebox[\linewidth]{\rule{5cm}{0.4pt}}

\noindent On: Friday 10th of October 2025

\noindent From: yuval.yarom@ruhr-uni-bochum.de

\noindent Title: Re: TCHES Volume 2026/2 - Long paper re-approval

\noindent Content:

Dear [[author name, redacted]],

Thank you for reaching out. We approve submission as a long paper with a page limit of 30 pages. Your approval ID is: CHES-206-2-018

When submitting, please make sure to:

* Note your approval ID (CHES-206-2-018) in the Comments to Editors-in-Chief field

* Mark the checkbox indicating a long paper

* Start the paper title with: "Long Paper:"

* Include a justification for a long paper either in the main submission or in the Supplementary material

Please note that this approval does not replace reviewers' discretion and we will respect reviewers' recommendation with respect to paper length.

Kind regards

Nele and Yuval


==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.46586/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

